Approximate Collapsed Gibbs Clustering with Expectation Propagation

We develop a framework for approximating collapsed Gibbs sampling in generative latent variable cluster models. Collapsed Gibbs is a popular MCMC method, which integrates out variables in the posterior to improve mixing. Unfortunately for many complex models, integrating out these variables is either analytically or computationally intractable. We efficiently approximate the necessary collapsed Gibbs integrals by borrowing ideas from expectation propagation. We present two case studies where exact collapsed Gibbs sampling is intractable: mixtures of Student-t's and time series clustering. Our experiments on real and synthetic data show that our approximate sampler enables a runtime-accuracy tradeoff in sampling these types of models, providing results with competitive accuracy much more rapidly than the naive Gibbs samplers one would otherwise rely on in these scenarios.

==> supp_scalemix.tex <==
This section provides the supplementary material for
Sec.~\ref{sec:scalemix} on Gaussian scale mixtures (GSM).
We provide the details on how to calculate the sufficient statistics of
$\mu, \Sigma$ required for our EP approximation.

We now present how to collapse out $\mu, \Sigma$,
approximating $p(\mu, \Sigma | y, z, w,r)$ with a normal inverse-Wishart.


This consists of estimating three quantities from the tilted distribution
(i) the normalizing constant $\tilde{Z}_i$,
(ii) the mean $\E_{\tilde{p}_i}[\mu]$, and
(iii) the second moment $\E_{\tilde{p}_i}[\mu \mu^T]$.

The normalizing constant (a.k.a. the likelihood approximation) is a weighted
average
\begin{equation}
    \tilde{Z}_i = 
    \int f(y_i \,  \, \mu, \Sigma, w) q(\mu \, | \, z_{-i}) \ d \mu
    = 
    \sum_{c = 1}^C \int w_c \cdot \mathcal{N}(y_i \, | \, \mu,\Sigma_c)
    \cdot \mathcal{N}(\mu \, | \, \mu_{-i}, \Sigma_{-i}) \ d\mu 
    =
    \sum_{c = 1}^C w_c \cdot \tilde{Z}_c 
    \enspace,
\end{equation}
where $\tilde{Z}_c$ is the normalizing constant treating only component $c$
as likelihood.
This is easy t do since component $c$ is a Gaussian, which is conjugate.

Similarly, the tilted-mean and second moments are weighted averages
\begin{align}
    \nonumber
    \E_{\tilde{p}_i}[\mu] &= 
    \int \mu \cdot \tilde{Z}_i^{-1} f(y_i \, | \, \mu, \Sigma, w)
    q(\mu \, | \, z_{-i}) \ d \mu 
    \\ \nonumber &=
    \sum_{c = 1}^C \frac{w_c \tilde{Z}_c}{\tilde{Z}_i} \int 
    \mu \cdot \underbrace{
        \tilde{Z}_c^{-1} \mathcal{N}(y_i \, | \, \mu,\Sigma_c)
        \cdot \mathcal{N}(\mu \, | \, \mu_{-i}, \Sigma_{-i})
    }_{\tilde{p}_c(\mu)} \ d\mu 
    \\ &=
    \sum_{c = 1}^C \frac{w_c \tilde{Z}_c}{\tilde{Z}_i} \, \E_{\tilde{p}_c}[\mu]
\end{align}
\begin{align}
    \nonumber
    \E_{\tilde{p}_i}[\mu \mu^T] &= 
    \int \mu\mu^T \cdot \tilde{Z}_i^{-1} f(y_i \, | \, \mu, \Sigma, w)
    q(\mu \, | \, z_{-i}) \ d \mu 
    \\ \nonumber &=
    \sum_{c = 1}^C \frac{w_c \tilde{Z}_c}{\tilde{Z}_i} \int 
    \mu\mu^T \cdot \underbrace{
        \tilde{Z}_c^{-1} \mathcal{N}(y_i \, | \, \mu,\Sigma_c)
        \cdot \mathcal{N}(\mu \, | \, \mu_{-i},\Sigma_{-i})
    }_{\tilde{p}_c(\mu)} \ d\mu 
    \\ &=
    \sum_{c = 1}^C \frac{w_c \tilde{Z}_c}{\tilde{Z}_i} \, 
    \E_{\tilde{p}_c}[\mu\mu^T] \enspace,
\end{align}
where $\tilde{p_c}$ is the posterior for $\mu$ treating only component $c$ as
the likelihood.




